Enhancing Traffic Safety with AI and 6G: Latency Requirements and Real-Time Threat Detection

The rapid digitalization of urban infrastructure opens the path to smart cities, where IoT-enabled infrastructure enhances public safety and efficiency. This paper presents a 6G and AI-enabled framework for traffic safety enhancement, focusing on real-time detection and classification of emergency vehicles and leveraging 6G as the latest global communication standard. The system integrates sensor data acquisition, convolutional neural network-based threat detection, and user alert dissemination through various software modules of the use case. We define the latency requirements for such a system, segmenting the end-to-end latency into computational and networking components. Our empirical evaluation demonstrates the impact of vehicle speed and user trajectory on system reliability. The results provide insights for network operators and smart city service providers, emphasizing the critical role of low-latency communication and how networks can enable relevant services for traffic safety.

==> BestPractice.tex <==


% \begin{itemize}
%     \item Geofence-based model for service discovery tailored explicitly for IoT applications;
%     \item Client-oriented discovery process with fine granularity considering the initial discovery and the runtime discovery;
%     \item Real-life evaluation testbed and representative use-case application from the field of emergency vehicles detection.
% \end{itemize}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{images/RTTgeo2.PNG} %
%     \caption{Schematic of MESDD discovery process aided by geofences.}%
%     \label{fig:schematicGeoRTT}%
% \end{figure}

% \begin{itemize}
%   \item \textbf{Step 1 -}\textbf{ Request DNS address of the intermediate code} is used to find the address of the intermediate code $\omega_{intermediate}$. The intermediate code (IM code) enables the execution of the discovery process on the client side. % which enables us to execute the discovery process.  

%   \par
%   \item \textbf{Step 2 -}\textbf{ Resolve DNS response} provides the resolved address of the intermediate code in the required format.
%   \par
%   \item \textbf{Step 3 - }\textbf{ Request to retrieve intermediate code} is used to access the IM code from the resolved DNS based on the address provided in Step 2.
% \end{itemize}

% %--------

% We define the service $\omega$ as a tuple: 
% \[ \omega = \left \{ In_\omega, Out_\omega \right \} \]
% where $In_\omega$ is a set of inputs required to invoke $\omega, Out_\omega$ is the set of outputs returned by $\omega$ after its execution.%, and $W$ is the set of all services available in the service registry.

% Furthermore, we define an instance $\iota$ of service as: 

% \[\iota = \left \{\lambda_1 .. \lambda_n  \right \} \]
% where $\lambda$ defines a Location Descriptor (LD) (see table \ref{wrap-tabname:1}). Each instance requires at least one LD.


% \begin{table}
% %\scalebox{0.95}{
% \begin{tabular}{clc}\\\toprule  
% level  & Location Descriptor & datacenter\\\midrule
% stage \#4 &D4.IS44.Klagenfurt.Kaernten.app.domain & Edge\\  \midrule
% stage \#3 &IS44.Klagenfurt.Kaernten.app.domain  & Edge\\  \midrule
% stage \#2 &Klagenfurt.Kaernten.app.domain & Fog\\  \midrule
% stage \#1 &Kaernten.app.domain & Cloud\\  \midrule

% \end{tabular}%}
% \caption{Hierarchical levels of domain representations and their corresponding datacenters.}\label{wrap-tabname:1}
% \end{table}


==> conclusion.tex <==
# this is my comment
